On the online path extension problem -- Location and routing problems in board games

We consider an online version of a longest path problem in an undirected and planar graph that is motivated by a location and routing problem occurring in the board game "Turn & Taxis". Path extensions have to be selected based on only partial knowledge on the order in which nodes become available in later iterations. Besides board games, online path extension problems have applications in disaster relief management when infrastructure has to be rebuilt after natural disasters. For example, flooding may affect large parts of a road network, and parts of the network may become available only iteratively and decisions may have to be made without the possibility of planning ahead. We suggest and analyse selection criteria that identify promising nodes (locations) for path extensions. We introduce the concept of tentacles of paths as an indicator for the future extendability. Different initialization and extension heuristics are suggested on compared to an ideal solution that is obtained by an integer linear programming formulation assuming complete knowledge, i.e., assuming that the complete sequence in which nodes become available is known beforehand. All algorithms are tested and evaluated on the original "Turn & Taxis" graph, and on an extended version of the "Turn & Taxis" graph, with different parameter settings. The numerical results confirm that the number of tentacles is a useful criterion when selecting path extensions, leading to near-optimal paths at relatively low computational costs.

==> ProblemAndDefinition_KK.tex <==
In this section, we introduce a mathematical terminology that facilitates the formulation of path extension problems. While some definitions and notation are tailored towards the board game ``Thurn \& Taxis'', most concepts are more generally applicable and are thus formulated in a general context.


\subsection{Paths, leafs, and tentacles}\label{subsec:tentac}


%To be able to formulate the considered optimization problem, we first need some basic definitions. Here, we have the standard definition of an undirected graph.

\kk{We first review some basic concepts from graph theory. For a general introduction into this topic, we refer to the textbooks of ...} \todo{Referenzen einfuegen}


Let $G:=(V,E)$ be a simple and undirected graph with \kk{node set $V=\{v_1,\dots,v_n\}$, i.e., $|V|=n$, and edge set $E=\{e_1,\dots,e_m\}$, i.e.,} $|E|=m$. \kk{To simplify the notation, we will often refer to a node by its respective index, i.e., $v_i=i$, $i=1,\dots,n$. \todo{Die Indizierung ist etwas schwierig; wir müssen in einem Path ja auf beliebige Knoten verweisen koennen; es geht also nicht $P=(v_1,\dots,v_\ell)$ oder so.} Each edge $e_k\in E$ is defined by its two end nodes, i.e., $e_k=(v_i,v_j)=(i,j)$ with $v_i,v_j\in V$ and $v_i\neq v_j$.}
Let $A=(a_{i,j})_{i=1,\dots ,n;\ j=1,\dots ,n}$ \kk{denote} the adjacency matrix of $G$.
Then the \emph{degree} of a node $v_i\in V$ is \kk{given by} $$\delta (v_{\kk{i}}):=\sum_{\kk{j}=1}^{\kk{n}} a_{\kk{ij}} .$$
We consider \kk{simple} paths in $G$ that are defined as ordered sequences of \kk{pairwise different} nodes \kk{and edges, respectively. More precisely, $P=(v_{i_1},\dots,v_{i_\ell})=(i_1,\dots,i_\ell)$ is a \emph{simple path} of \emph{length} $\ell(P)=\ell$ if}
$(\kk{i_j,i_{j+1}})\in E$ for all $\kk{j}\in\{ 1,\dots ,\kk{\ell}-1\}$ and $\kk{i_j\neq i_k}$ for all $j\neq k$.\todo{Klassisch wird dieLaenge glaube ich ueber die Zahl der Kanten definiert.}

\kk{In this paper, we are interested in the iterative extension of simple paths by additional nodes with the ultimate goal of generating longest paths without node repetitions. In the context of the game Thurn \& Taxis, such extensions have to be made based on partial knowledge on the set of available nodes since in each iteration only a subset of nodes is visible and additional nodes become available only in later iterations. Other possible applications of such \emph{online path extension problems} may occur, for example, when planning recovery operations after natural disasters that cut off the majority of roads in a transportation network, where roads (and thus nodes) become available only iteratively. Throughout this paper, we assume that (sub-)paths $P=(i_1,\dots,i_\ell)$ can only be extended at their end-nodes, i.e., at either of the two nodes $i_1$ or $i_\ell$. In such contexts, the \emph{prolongation potential} of a current (sub-)path plays a decisive role for the (iterative) path extension. Indeed, when selecting the next node such that, based on the partial knowledge available, \emph{many} further extensions of the path are known to be feasible in consecutive iterations, it is probably more likely that a long path can be constructed than when choosing a node that allows for only few extensions. This motivates the definition of \emph{tentacles} of a path.}

\begin{definition}[Tentacles of a path]
    Let $G=(V,E)$ be a \kk{simple} graph and \kk{let} $P=(\kk{i}_1,\dots ,\kk{i}_{\kk{\ell}})$ be a \kk{simple} path in $G$. Then the \emph{tentacles} of $P$ are defined as $N_P:=\{ \kk{k}\in V\ :\ \kk{k}\notin P \text{ and } ( (\kk{k},\kk{i}_1)\in E \text{ or } (\kk{k},\kk{i}_{\kk{\ell}})\in E\}$. The \emph{number of tentacles} of $P$ is given by $$\delta_P \kk{:=} |N_P|.$$
\end{definition}

\kk{See Figure~\ref{Ex:TentacleDef} for an illustration of a simple path and its tentacles.}

\begin{figure}
    \small
    \centering
    \begin{tikzpicture}[scale=0.6,every node/.style={draw=black,circle,font=\footnotesize,inner sep=1pt,minimum size=10pt}]
    \node[dashed] (1) at (2,0) {};
    \node (2) at (4,0) {};
    \node (3) at (6,0) {};
    \node[dotted] (4) at (8,0) {};
    \node[dashed] (5) at (0,-2) {};
    \node (6) at (2,-2) {};
    \node[dashed] (7) at (4,-2) {};
    \node (8) at (6,-2) {};
    \node[dashed] (9) at (8,-2) {};
    \node[dotted] (10) at (4,-4) {};
    \node[dashed] (11) at (6,-4) {};
    \node[dotted] (12) at (8,-4) {};
    \node[dashed] (13) at (2,-4) {};
    \node[dotted] (14) at (4,-6) {};
    \node[dotted] (15) at (6,-6) {};
    \node[dotted] (16) at (4,2) {};
    \node[dotted] (17) at (6,2) {};
    \node[dotted] (18) at (8,2) {};
    \filldraw[black] (2) circle (10pt);
    \filldraw[black] (3) circle (10pt);
    \filldraw[black] (6) circle (10pt);
    \filldraw[black] (8) circle (10pt);
    \draw[-,thick] (2) to (3);
    \draw[-,thick] (2) to (6);
    \draw[-,thick] (3) to (8);
    \draw[dashed] (6) to (7);
    \draw[dotted] (7) to (10);
    \draw[dotted] (7) to (11);
    \draw[dotted] (10) to (11);
    \draw[dotted] (2) to (6);
    \draw[dashed] (8) to (11);
    \draw[dashed] (7) to (8);
    \draw[dotted] (1) to (2);
    \draw[dashed] (1) to (6);
    \draw[dotted] (2) to (16);
    \draw[dotted] (3) to (4);
    \draw[dotted] (3) to (17);
    \draw[dotted] (3) to (18);
    \draw[dashed] (5) to (6);
    \draw[dashed] (6) to (13);
    \draw[dashed] (8) to (9);
    \draw[dotted] (9) to (11);
    \draw[dotted] (10) to (13);
    \draw[dotted] (10) to (14);
    \draw[dotted] (11) to (12);
    \draw[dotted] (11) to (14);
    \draw[dotted] (11) to (15);
    \end{tikzpicture}
    \caption{\kk{A simple graph $G=(V,E)$, where $V$ comprises all dotted, dashed and filled nodes, with a simple path $P$ (filled nodes). The dashed nodes are the tentacles of $P$ and hence $\delta_P=6$.}\label{Ex:TentacleDef}}
\end{figure}


\begin{lemma}\label{lemma:bounds}
    Let $G=(V,E)$ be a \kk{simple} graph and \kk{let} $P=(\kk{i}_1,\dots ,\kk{i}_{\kk{\ell}})$ be a \kk{simple} path in $G$ with \kk{length} $\ell(P)=\kk{\ell}$. \kk{Then} the following properties hold:
    \begin{enumerate}
        \item $\delta_P\leq |V|-\kk{\ell}$;
        \item if $\kk{\ell}=1$, \kk{then} $\delta_P=\delta(\kk{i}_1)$;
        \item if $\kk{\ell}\geq 2$, \kk{then} $\delta_P\leq \delta(\kk{i}_1)+\delta(\kk{i}_{\kk{\ell}})-2$; \kk{this bound is tight when $G$ is a tree;}
        \item \kk{If $\ell\geq 2$, then $\delta_P \geq \max\{\delta(i_1),\delta(i_\ell)\}-\ell$}.
        %\item $\delta_P\geq \delta(v_1)+\delta(v_k)-\min\lbrace \delta (v_1),k-1\rbrace - \min\lbrace \delta (v_k),k-1\rbrace$ Die Formel ist falsch.
        %\item In gridgraphs: $\delta_P\leq 6$
        %\item In octographs: $\delta_P\leq 14$
    \end{enumerate}
\end{lemma}
\begin{proof}
    The statements follow directly from the definition.
\end{proof}

\kk{Note that the bound in Lemma~\ref{lemma:bounds} (4) is also tight, for example, when $\delta(i_1)=\delta(i_\ell)$, both nodes $i_1$ and $i_\ell$ are adjacent to all nodes in $P$, and all other nodes that are adjacent to $i_1$ are also adjacent to $i_\ell$ (and vice versa).}

\subsection{Available nodes and extension tuples}

\kk{In this section we focus on the particular setting in the game Thurn \& Taxis. Here, path extensions can only be chosen from a finite selection of available nodes that has constant size during the course of the game. Such selections will be stored using vectors, or tuples, of nodes.  Selections may contain duplicates, i.e., nodes may occur several times in a selection, which reduces the number of actual choices. Whenever one node is selected as an extension, another node is added to the selection and hence becomes  available for the next iteration.} 
The three following definitions are needed to mathematically describe one instance of the \kk{resulting game, which may be interpreted as an online path extension problem.} 


\begin{definition}[Initial tuple and initial set]
    \kk{Let} $N_D\in\mathbb{N}$ denote the \emph{number of duplicates of every node}. \kk{Moreover,} let $(\kk{i}_1,\dots,\kk{i}_c)$ with $\kk{i_k}\in V$, $\kk{k}=1,\dots ,c$, be an \emph{initial tuple} \kk{of} \emph{size} $c\in\mathbb{N}$, referred to as \emph{initial $c$-tuple} in the following. Note that $\kk{i_j = i_k,\ j\neq k}$ is not forbidden, but there must not be more than $N_D$ versions of the same node in this tuple.
    $\Vinit:=\lbrace \kk{i}_1,\dots ,\kk{i}_c \rbrace$ is called \emph{initial $c$-set}.
\end{definition}

\kk{The initial $c$-set specifies the set of nodes that are available in the first iteration of the game. Hence, the first node of the path has to be selected from the set $\Vinit$. Moreover, we assume that all nodes in $V$ occur exactly $N_D$ times in a deck of cards (representing nodes) that is given and fixed from the beginning of the game, however, unknown to the players. This node deck can be represented by a vector of length $n\cdot N_D$, that results from combining an initial $c$-tuple with an appropriate \emph{extension tuple}. In this context, the extension tuple contains the information on possible path extensions during later iterations of the game.} 
    
\begin{definition}[Extension tuple]
    Let \kk{$d:=n\cdot N_D-c$ denote the total number of remaining cards in a given node deck that are not contained in the initial $c$-tuple. Then}  $(\kk{j}_1,\dots ,\kk{j}_d)$ with $\kk{j_k}\in V$, $\kk{k}= 1,\dots ,d$, is called an \emph{extension tuple} of size $d$, also referred to as \emph{ordered extension $d$-tuple}, \kk{if the total number of duplicates is bounded by $N_D$ for every node $i\in V$, $i=1,\dots,n$. In other words,}
    $\kk{j_k=j_s, k\neq s}$ is not forbidden, but there can be at most $N_D$ \kk{copies} of the same node in \kk{an extension} tuple.
\end{definition}

\kk{To avoid confusion, we will refer to nodes from an initial tuple by $i_k$, $k\in\{1,\dots,c\}$, while the nodes from an extension tuple will be denoted by $j_k$, $k\in\{1,\dots,d\}$.} \todo{Das muss noch umgesetzt werden. Knoten koennen sonst nicht richtig zugeordnet werden.}

\kk{Combining an initial $c$-tuple with an extension tuple thus yields a deck of exactly $n\cdot N_D$ cards. Note that, while the order of nodes in an extension tuple is decisive for the order in which new nodes become available during the course of the game, the order of nodes not relevant for the initial $c$-tuple since all of its nodes become available simultaneously at the initialization of the game. An instance of the game can now be defined using \emph{feasible settings} that combine an initial $c$-tuple with an appropriate extension tuple such that each node or card, respectively, occurs exactly $N_D$ times.}  

\begin{definition}[Feasible setting]
    A \emph{feasible setting} consists of an initial $c$-tuple and an ordered extension $d$-tuple, such that $d=|V|\cdot N_D-c$ holds and \kk{such} that there are exactly $N_D$ \kk{copies} of every node in the combination of both tuples.
    A \emph{$(c,N_D)$-setting} is a family of all feasible settings \kk{for a given problem size}. %with an intial $c$-tuple and an ordered extension $d$-tuple.
\end{definition}


Now we \kk{can describe an instance of the online path extension problem.} Assume \kk{that} a \kk{simple} graph and a feasible \kk{$(c,N_D)$-}setting \kk{are} given \kk{consisting of an initial tuple $\Vinit=\{i_1,\dots,i_c\}$ and and extension tuple $\{j_1,\dots,j_d\}$. Then} we want to \kk{find a simple path $P$ of maximum length that is generated iteratively according to the following procedure:}
\begin{enumerate}
    \item Pick one node $v_{\text{start}}$ belonging to the initial tuple. Set $k=1$. Set $P_0=(v_{\text{start}})$.
    \item Pick one node $v_{\text{new}}\kk{\in}\Vinit\cup\lbrace \kk{j}_1,\dots,\kk{j}_k \rbrace$ which is adjacent to at least one end node of $P_{k-1}$. If there is no adjacent node: Stop.
    \item Add $v_{\text{new}}$ at the end or at the beginning of the path $P_{k-1}$ (such that it is adjacent to that endpoint) to create $P_k$. Increase $k$ by one.
    \item Continue with (2) or end the procedure.
\end{enumerate}
\kk{Note that during this procedure,} theextension tuple is \kk{only partly known. Indeed,} in step (1) there is no information about the order of the extension tuple and in step (2) only the information on the first $k$ elements (where $k$ is the length of the \kk{current} path) of the extension tuple is \kk{known.}

\subsection{Interpretation in terms of the game "Thurn and Taxis"}

One application corresponding to the aforementioned definitions and optimization problem is a simplified one player version of the board game "Thurn and Taxis". In this game the players operate on a graph with $22$ nodes which represent different cities in southern Germany, Austria, Switzerland, Czechia and Poland. The game comes to an end if one player manages to build $20$ postal offices - there must be not more than one postal office of every player per city. It is possible to build such a postal office in a city if the corresponding node is used in the path that a player just finished. It is possible to finish a path after adding another node to it. If you decide to continue the path instead, you are forced to prolong the path in the next round. If you fail to do so, your path is lost and you have to start a new one. There are $6$ cards on display from which you can choose one to start or prolong your path. To prolong you path you have to add the new card to the "left" or "right" end of your path, which is only possible if the node at the end is adjacent to the node you want to add - so it is forbidden to squeeze a node between to nodes in the middle of your path.


The number of duplicates denotes how many cards of every city are in the set of cards. There are three copies of every city in the set of cards of the original "Thurn and Taxis". A feasible setting is a complete stack of cards, divided into a part that is visible at the beginning of a game (the initial tuple) and another part that is drawn as the game progresses (the extension tuple). We aim to heuristically model the decision process of a single player variant of "Thurn and Taxis".\\
First one has to choose a card of a city from the initial tuple to initialize a path while not having any information of the order of the cards in the extension tuple. After that you are able to choose a card from the initial tuple or the first $k$ elements of the extension tuple, where $k$ is the length of the so far computed path, while not having any information of the order of the cards in the expansion tuple apart from the first $k$ cards.
\todo{more text. gogo}




==> ProblemAndDefinition_KK2.tex <==
In this section, we introduce a mathematical terminology that facilitates the formulation of path extension problems. While some definitions and notation are tailored towards the board game ``Thurn \& Taxis'', most concepts are more generally applicable and are thus formulated in a general context.


\subsection{Paths, leafs, and tentacles}\label{subsec:tentac}


%To be able to formulate the considered optimization problem, we first need some basic definitions. Here, we have the standard definition of an undirected graph.

\kk{We first review some basic concepts from graph theory. For a general introduction into this topic, we refer to the textbooks of ...} \todo{Referenzen einfuegen}


Let $G:=(V,E)$ be a simple and undirected graph with node set $V=\{v_1,\dots,v_n\}$, i.e., $|V|=n$, and edge set $E=\{e_1,\dots,e_m\}$, i.e., $|E|=m$. To simplify the notation, we will often refer to a node by its respective index, i.e., $v_i=i$, $i=1,\dots,n$.  Each edge $e_k\in E$ is defined by its two end nodes, i.e., $e_k=(v_i,v_j)=(i,j)$ with $v_i,v_j\in V$ and $v_i\neq v_j$.
Let $A=(a_{i,j})_{i=1,\dots ,n;\ j=1,\dots ,n}$ denote the adjacency matrix of $G$.
Then the \emph{degree} of a node $v_i\in V$ is given by $$\delta (v_{i}):=\sum_{j=1}^{n} a_{ij} .$$
We consider simple paths in $G$ that are defined as ordered sequences of pairwise different nodes and edges, respectively. More precisely, $P=\Path $ is a \emph{simple path} of \emph{node length} $\ell(P)=\ell$ if $(l,l+1)\in E$ for all $l\in\{ 1,\dots ,\ell-1\}$ and $p_l\neq p_k$ for all $l\neq k$. Note that we do not define the length of a path using the number of edges but the number of contained nodes. Because of that we are referring to the \emph{node length} of a path instead of its length.

In this paper, we are interested in the iterative extension of simple paths by additional nodes with the ultimate goal of generating longest paths without node repetitions. In the context of the game Thurn \& Taxis, such extensions have to be made based on partial knowledge on the set of available nodes since in each iteration only a subset of nodes is visible and additional nodes become available only in later iterations. Other possible applications of such \emph{online path extension problems} may occur, for example, when planning recovery operations after natural disasters that cut off the majority of roads in a transportation network, where roads (and thus nodes) become available only iteratively. Throughout this paper, we assume that (sub-)paths $P=(i_1,\dots,i_\ell)$ can only be extended at their end-nodes, i.e., at either of the two nodes $i_1$ or $i_\ell$. In such contexts, the \emph{prolongation potential} of a current (sub-)path plays a decisive role for the (iterative) path extension. Indeed, when selecting the next node such that, based on the partial knowledge available, \emph{many} further extensions of the path are known to be feasible in consecutive iterations, it is generally more likely that a long path can be constructed than when choosing a node that allows for only few extensions. This motivates the definition of \emph{tentacles} of a path.

\begin{definition}[Tentacles of a path]
    Let $G=(V,E)$ be a simple graph and let $P=\Path $ be a simple path in $G$. Then the \emph{tentacles} of $P$ are defined as $\tentacleP:=\{ v\in V\ :\ v\notin P \text{ and } ( (v,p_1)\in E \text{ or } (v,p_{\ell})\in E\}$. The \emph{number of tentacles} of $P$ is given by $$\delta_P := |\tentacleP|.$$
\end{definition}

See Figure~\ref{Ex:TentacleDef} for an illustration of a simple path and its tentacles.

\begin{figure}
    \small
    \centering
    \begin{tikzpicture}[scale=0.6,every node/.style={draw=black,circle,font=\footnotesize,inner sep=1pt,minimum size=10pt}]
    \node[dashed] (1) at (2,0) {};
    \node (2) at (4,0) {};
    \node (3) at (6,0) {};
    \node[dotted] (4) at (8,0) {};
    \node[dashed] (5) at (0,-2) {};
    \node (6) at (2,-2) {};
    \node[dashed] (7) at (4,-2) {};
    \node (8) at (6,-2) {};
    \node[dashed] (9) at (8,-2) {};
    \node[dotted] (10) at (4,-4) {};
    \node[dashed] (11) at (6,-4) {};
    \node[dotted] (12) at (8,-4) {};
    \node[dashed] (13) at (2,-4) {};
    \node[dotted] (14) at (4,-6) {};
    \node[dotted] (15) at (6,-6) {};
    \node[dotted] (16) at (4,2) {};
    \node[dotted] (17) at (6,2) {};
    \node[dotted] (18) at (8,2) {};
    \filldraw[black] (2) circle (10pt);
    \filldraw[black] (3) circle (10pt);
    \filldraw[black] (6) circle (10pt);
    \filldraw[black] (8) circle (10pt);
    \draw[-,thick] (2) to (3);
    \draw[-,thick] (2) to (6);
    \draw[-,thick] (3) to (8);
    \draw[dashed] (6) to (7);
    \draw[dotted] (7) to (10);
    \draw[dotted] (7) to (11);
    \draw[dotted] (10) to (11);
    \draw[dotted] (2) to (6);
    \draw[dashed] (8) to (11);
    \draw[dashed] (7) to (8);
    \draw[dotted] (1) to (2);
    \draw[dashed] (1) to (6);
    \draw[dotted] (2) to (16);
    \draw[dotted] (3) to (4);
    \draw[dotted] (3) to (17);
    \draw[dotted] (3) to (18);
    \draw[dashed] (5) to (6);
    \draw[dashed] (6) to (13);
    \draw[dashed] (8) to (9);
    \draw[dotted] (9) to (11);
    \draw[dotted] (10) to (13);
    \draw[dotted] (10) to (14);
    \draw[dotted] (11) to (12);
    \draw[dotted] (11) to (14);
    \draw[dotted] (11) to (15);
    \end{tikzpicture}
    \caption{A simple graph $G=(V,E)$, where $V$ comprises all dotted, dashed and filled nodes, with a simple path $P$ (filled nodes). The dashed nodes are the tentacles of $P$ and hence $\delta_P=6$.\label{Ex:TentacleDef}}
\end{figure}


\begin{lemma}\label{lemma:bounds}
    Let $G=(V,E)$ be a simple graph and let $P=\Path$ be a simple path in $G$ with node length $\ell(P)=\ell$. Then the following properties hold:
    \begin{enumerate}
        \item $\delta_P\leq |V|-\ell$;
        \item if $\ell=1$, then $\delta_P=\delta(p_1)$;
        \item if $\ell\geq 2$, then $\delta_P\leq \delta(p_1)+\delta(p_{\ell})-2$; this bound is tight when $G$ is a tree;
        \item If $\ell\geq 2$, then $\delta_P \geq \max\{\delta(p_1),\delta(p_\ell)\}-\ell$.
        %\item $\delta_P\geq \delta(v_1)+\delta(v_k)-\min\lbrace \delta (v_1),k-1\rbrace - \min\lbrace \delta (v_k),k-1\rbrace$ Die Formel ist falsch.
        %\item In gridgraphs: $\delta_P\leq 6$
        %\item In octographs: $\delta_P\leq 14$
    \end{enumerate}
\end{lemma}
\begin{proof}
    The statements follow directly from the definition.
\end{proof}

Note that the bound in Lemma~\ref{lemma:bounds} (4) is also tight, for example, when $\delta(p_1)=\delta(p_\ell)$, both nodes $p_1$ and $p_\ell$ are adjacent to all nodes in $P$, and all other nodes that are adjacent to $p_1$ are also adjacent to $p_\ell$ (and vice versa).

\subsection{Available nodes and extension tuples}

In this section we focus on the particular setting in the game Thurn \& Taxis, which may be interpreted as an online path extension problem. Here, path extensions can only be chosen from a finite selection of available nodes that has constant size during the course of the game. Such selections will be stored using vectors, or tuples, of nodes.  Selections may contain duplicates, i.e., nodes may occur several times in a selection, which reduces the number of actual choices. Whenever one node is selected as an extension, another node is added to the selection and hence becomes  available for the next iteration.
The three following definitions are needed to mathematically describe one instance of the resulting game.


\begin{definition}[Initial tuple and initial set]
    Let $\Dupl\in\mathbb{N}$ denote the \emph{number of duplicates of every node}. Moreover, let $(i_1,\dots,i_c)$ with $i_k\in V$, $k=1,\dots ,c$, be an \emph{initial tuple} of \emph{size} $c\in\mathbb{N}$, referred to as \emph{initial $c$-tuple} in the following. Note that $i_l = i_k,\ l\neq k$ is not forbidden, but there must not be more than $\Dupl$ versions of the same node in this tuple.
    $\Vinit:=\lbrace i_1,\dots ,i_c \rbrace$ is called \emph{initial $c$-set}.
\end{definition}

The initial $c$-set specifies the set of nodes that are available in the first iteration of the game. Hence, the first node of the path has to be selected from the set $\Vinit$. Moreover, we assume that all nodes in $V$ occur exactly $\Dupl$ times in a deck of cards (representing nodes) that is given and fixed from the beginning of the game, however, unknown to the players. This node deck can be represented by a vector of length $n\cdot \Dupl$, that results from combining an initial $c$-tuple with an appropriate \emph{extension tuple}. In this context, the extension tuple contains the information on possible path extensions during later iterations of the game.
    
\begin{definition}[Extension tuple]
    Let $d:=n\cdot \Dupl-c$ denote the total number of remaining cards in a given node deck that are not contained in the initial $c$-tuple. Then  $(j_1,\dots ,j_d)$ with $j_k\in V$, $k= 1,\dots ,d$, is called an \emph{extension tuple} of size $d$, also referred to as \emph{ordered extension $d$-tuple}, if the total number of duplicates is bounded by $\Dupl$ for every node $i\in V$, $i=1,\dots,n$. In other words,
    $j_k=j_s, k\neq s$ is not forbidden, but there can be at most $\Dupl$ copies of the same node in an extension tuple.
\end{definition}

\todo{Bemerkung einfügen: Inital tuple + extension tuple als "ganzen" Stapel definieren, anstatt einzeln.}

To avoid confusion, we will refer to nodes from an initial tuple by $i_k$, $k\in\{1,\dots,c\}$, while the nodes from an extension tuple will be denoted by $j_k$, $k\in\{1,\dots,d\}$.\todo{Noch einmal überall überprüfen, ob es richtig angepasst ist}

Combining an initial $c$-tuple with an extension tuple thus yields a deck of exactly $n\cdot \Dupl$ cards. Note that, while the order of nodes in an extension tuple is decisive for the order in which new nodes become available during the course of the game, the order of nodes is not relevant for the initial $c$-tuple since all of its nodes become available simultaneously at the initialization of the game. An instance of the game can now be defined using \emph{feasible settings} that combine an initial $c$-tuple with an appropriate extension tuple such that each node or card, respectively, occurs exactly $\Dupl$ times.

\begin{definition}[Feasible setting]
    A \emph{feasible setting} consists of an initial $c$-tuple and an ordered extension $d$-tuple, such that $d=|V|\cdot \Dupl-c$ holds and such that there are exactly $\Dupl$ copies of every node in the combination of both tuples.
    A \emph{$(c,\Dupl)$-setting} is a family of all feasible settings for a given problem size. %with an intial $c$-tuple and an ordered extension $d$-tuple.
\end{definition}


Now we can describe an instance of the online path extension problem. Assume that a simple graph and a feasible $(c,\Dupl)$-setting are given consisting of an initial tuple $(i_1,\dots,i_c)$ and and extension tuple $(j_1,\dots,j_d)$. Then we want to find a simple path $P$ of maximum node length that is generated iteratively according to the following procedure:
\begin{enumerate}
    \item Pick one node $\startp$ belonging to the initial tuple. Set $k=1$. Set $P_0=(\startp)$.
    \item Pick one node $\extp\in\Vinit\cup\lbrace j_1,\dots,j_k \rbrace$ which is adjacent to at least one end node of $P_{k-1}$. If there is no such node: Stop.
    \item Add $\startp$ at the end or at the beginning of the path $P_{k-1}$ (such that it is adjacent to that endpoint) to create $P_k$. Increase $k$ by one.
    \item Continue with (2) or end the procedure.
\end{enumerate}
Note that during this procedure, the extension tuple is only partly known. Indeed, in step (1) there is no information about the order of the extension tuple and in step (2) only the information on the first $k$ elements (where $k$ is the node length of the current path) of the extension tuple is known.

\subsection{Interpretation in terms of the game "Thurn and Taxis"}

One application of an online path extension problem is a simplified one-player version of the board game ``Thurn and Taxis''. In this game, players operate on a graph with $22$ nodes which represent different cities in southern Germany, Austria, Switzerland, Czechia and Poland. The game comes to an end whenever one player manages to build $20$ postal offices, under the constraint that there can not be more than one postal office per player per city. In order to build postal offices, players iteratively extend paths (that represent potential postal routes). In each iteration, a player has to add an additional node to his or her current path. The player can then decide to ``close'' this path and build postal offices in all of its nodes, or to try to further extend the path in the next round. The latter choice bears some risk: If it turns out impossible to extend the path in the next round, the path has to be discarded and no postal offices can be build on any of its nodes. The player then has to start over with a new path.  There are always six cards on display from which a player can select one node to start or to extend his or her path. To extend a path, the next node must be added to the first or to the last node of the current path.


The number of duplicates indicates how many cards of every city are in the set of cards. There are three copies of every city in the set of cards of the original game ``Thurn and Taxis'', i.e., $\Dupl=3$ in the original setting. A feasible setting corresponds to a complete stack of cards, divided into a part that is visible at the beginning of a game (the initial tuple) and another part that is drawn as the game progresses (the extension tuple). We aim to heuristically model the decision process of a single player variant of "Thurn and Taxis".

In the first iteration of a single-player version of this game, the player has to choose a card of a city from the initial tuple to initialize a path while not having any information on the order of the cards in the extension tuple. In all later iterations, the player can select a card from the initial tuple or from the first $k$ elements of the extension tuple, where $k$ is the total node length of the paths computed so far. Again, no information on the order of the remaining cards in the extension tuple (apart from the first $k$ cards) is available to the player.

In this paper, we focus on the generation of the \emph{first} path and stop the path construction whenver no additional node can be added to one of its end nodes. We consider a single-player version in the sense that there is no competition, i.e., there are no other players competing about the available cards. Moreover, we evaluate the final path node length without requiring the player to make a stopping decision.



